Neighbor Oblivious Learning (NObLe) for Device Localization and Tracking

On-device localization and tracking are increasingly crucial for various applications. Along with a rapidly growing amount of location data, machine learning (ML) techniques are becoming widely adopted. A key reason is that ML inference is significantly more energy-efficient than GPS query at comparable accuracy, and GPS signals can become extremely unreliable for specific scenarios. To this end, several techniques such as deep neural networks have been proposed. However, during training, almost none of them incorporate the known structural information such as floor plan, which can be especially useful in indoor or other structured environments. In this paper, we argue that the state-of-the-art-systems are significantly worse in terms of accuracy because they are incapable of utilizing these essential structural information. The problem is incredibly hard because the structural properties are not explicitly available, making most structural learning approaches inapplicable. Given that both input and output space potentially contain rich structures, we study our method through the intuitions from manifold-projection. Whereas existing manifold based learning methods actively utilized neighborhood information, such as Euclidean distances, our approach performs Neighbor Oblivious Learning (NObLe). We demonstrate our approach's effectiveness on two orthogonal applications, including WiFi-based fingerprint localization and inertial measurement unit(IMU) based device tracking, and show that it gives significant improvement over state-of-art prediction accuracy.

==> manifold.tex <==
\section{Why Deep Multi-Label is Equivalent to Manifold Learning}
Multidimensional scaling (MDS) objective is utilized for several metric manifold learning algorithms such as Isomap. Consider the objective function of MDS,
\begin{equation*}
    f(Z) = \sum_{i=1}^n \sum_{j=1+i}^n ( ||z_i - z_j|| - ||x_i - x_j||)^2.
\end{equation*}
The idea is to learn vector $Z$ such the manifold structural relationship between data points is preserved. In this loss function, close neighbors, in the manifold distance, are encouraged to stay close in the reconstructed space and far away points are encouraged to stay far away. 

In our formulation of \noble, we use binary cross-entropy loss function for multi-label classification, defined as
\begin{align*}
& J(W, (h_c,\hat{h}_c)) = \\  & \qquad\sum_{i=1}^N \sum_{c=1}^K -h_c \log (\hat{h}_c) - (1-h_c) \log (1-\hat{h}_c),
\end{align*}
where $K$ is the number of classes, $h_c \in \{0,1\}$ indicates the true class, and $\hat{h}_c$ is the sigmoid function
\begin{equation*}
    \hat{h}_c = (1 + \exp(-w_c^{(\ell)\top} z^{(\ell)}_i)^{-1},
\end{equation*}
where $\ell$ denotes the last layer of the neural network, $w_c^{\ell}$ denotes for the weight vector for class c at $\ell$ layer, $z_i$ denotes for the layer layer logits given input $x_i$. 

It is known that in a deep network, the last but one (penultimate) layer output can be interpreted as learned embedding from input features. 
Thus, we focus our analysis on the last layer $\ell$. For simplicity, suppose $w$ and $z$ are normalized (i.e., $w^\top w = z^\top z = 1$), we can rewrite $\hat{h}$ from an inner product to the Euclidean distance form as
\begin{equation*}
    \hat{h}_c = (1 + \exp(1/2||w_c^{(\ell)} - z^{(\ell)}_i||^2 - 1))^{-1}.
\end{equation*}
For a given $c$, minimizing the cross-entropy loss will result in a setting to $w_c^{(\ell)}$ such that $||w_c^{(\ell)} - z^{(\ell)}_i||$ for the true class is minimized (cf. false class is maximized).
\begin{proposition}
Let $W$ be the result of minimized cross-entropy objective such that, at inference (or prediction) time, the following holds for two embedding $z_i$ and $z_j$
\begin{equation*}
||w_c^{(\ell)} - z^{(\ell)}_i||^2 \leq \lambda \qquad \text{and} \qquad
||w_c^{(\ell)} - z^{(\ell)}_j||^2 \leq \lambda.
\end{equation*}
Then, by triangle inequality, we have $||z^{(\ell)}_i - z^{(\ell)}_j||^2 \leq 2\lambda$, where $\lambda$ is a small constant.
\end{proposition}

From a manifold perspective, embedding from last layer can be interpreted as reconstructed embedding. Consider $z_i$ as embedding given input $x_i$, $z_j$ as embedding given input $x_j$. If $x_i$, $x_j$ are near neighbors, then by our neighbor oblivious formulation, there must exists a few common class labels, which both of them should predict. Let the weights associated with the common class be denoted by $w_{common}$. Using the above proposition with $w_{common}$,  $z_i$, $z_j$ is expected to be close. This resembles the objective function of MDS under our neighbor oblivious formulation where distance in the input space between $x_i$ and $x_j$ is not considered.

